Experimental Findings on the Sources of Detected Unrecoverable Errors in GPUs

We investigate the sources of Detected Unrecoverable Errors (DUEs) in GPUs exposed to neutron beams. Illegal memory accesses and interface errors are among the more likely sources of DUEs. ECC increases the launch failure events. Our test procedure has shown that ECC can reduce the DUEs caused by Illegal Address access up to 92% for Kepler and 98% for Volta.

==> src/due_source_table.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{graphicx}
\begin{table*}[]
	\caption{The NVIDIA API DUE motivation under the beam. All errors in this table were observed at least once in the beam experiments. Adapted from~\cite{cudaToolkitDocumentation}}
	\label{tab_due_source_api}
	\resizebox{\textwidth}{!}{%
		\begin{tabular}{|l|l|}
			\hline
			\textbf{CUDA API Error}                                                                & \textbf{Detailed explanation}                                                                                                                                                                                                                              \\ \hline
			\textbf{Devices Unavailable}                                                            & \begin{tabular}[c]{@{}l@{}}The device became unavailable both when  the GPU mode became Exclusive or Prohibited, or the\\  previous kernel execution did not release the used resources, and the device is "falsely" full.\end{tabular}                    \\ \hline
			\textbf{Illegal Instruction}                                                            & When an illegal instruction happens during the kernel execution, leaving the process in an inconsistent status.                                                                                                                                            \\ \hline
			\textbf{\begin{tabular}[c]{@{}l@{}}Illegal Address or\\ Misaligned Address\end{tabular}} & The address used in a Load or Store instruction does not point to a valid memory address or is not aligned.                                                                                                                                                \\ \hline
			\textbf{Initialization Error}                                                           & The CUDA driver failed to initialize, making it impossible for the API continues.                                                                                                                                                                          \\ \hline
			\textbf{\begin{tabular}[c]{@{}l@{}}Invalid Device or\\ No Device\end{tabular}}           & The selected device by the CPU is invalid, or the CUDA driver detects no device.                                                                                                                                                                           \\ \hline
			\textbf{Invalid PC}                                                                     & One of the kernel program counters got corrupted consequentially became invalid.                                                                                                                                                                           \\ \hline
			\textbf{Invalid Address Space}                                                           & \begin{tabular}[c]{@{}l@{}}A CUDA kernel can operate in different spaces of memories (i.e., global, shared, or local). This error happens\\  when an instruction that belongs to a specific memory space try to operate in a different one\end{tabular}    \\ \hline
			\textbf{Memory Allocation}                                                              & The CUDA API is not able to allocate memory on GPU.                                                                                                                                                                                                        \\ \hline
			\textbf{System Crash}                                                                   & \begin{tabular}[c]{@{}l@{}}It is a DUE triggered by our setup software or hardware watchdog. Then the DUE source could not be traced \\ or is generally unknown.\end{tabular}                                                                              \\ \hline
			\textbf{ECC Uncorrectable}                                                              & When the Error Correction Code detects more than 1 bit of flip in the memories, it cannot be corrected.                                                                                                                                                    \\ \hline
			\textbf{Launch Failure}                                                                 & \begin{tabular}[c]{@{}l@{}}This error occurs when the CPU tries to launch a kernel and fails. There are many reasons that it could happen, \\ such as dereferencing an invalid device pointer and accessing out of bounds shared memory, etc.\end{tabular} \\ \hline
			\textbf{Hardware Stack Error}                                                            & \begin{tabular}[c]{@{}l@{}}This error happens due to an error in the call stack during kernel execution, generally due to stack corruption \\ or exceeding the stack size limit.\end{tabular}                                                              \\ \hline
			\textbf{Invalid Value}                                                                  & \begin{tabular}[c]{@{}l@{}}This indicates that some parameters passed to the GPU are out of the acceptable range of values. \\ For example, more threads than the GPU supports.\end{tabular}                                                               \\ \hline
		\end{tabular}%
	}
\end{table*}

